$K_L-K_S$ mass difference from lattice QCD

We report on the first complete calculation of the $K_L-K_S$ mass difference, $\Delta M_K$, using lattice QCD. The calculation is performed on a 2+1 flavor, domain wall fermion ensemble with a 330MeV pion mass and a 575 MeV kaon mass. We use a quenched charm quark with a 949 MeV mass to implement Glashow-Iliopoulos-Maiani cancellation. For these heavier-than-physical particle masses, we obtain $\Delta M_K =3.19(41)(96)\times 10^{-12}$ MeV, quite similar to the experimental value. Here the first error is statistical and the second is an estimate of the systematic discretization error. An interesting aspect of this calculation is the importance of the disconnected diagrams, a dramatic failure of the OZI rule.

==> changes.tex <==
Changes to v4:
--------------------------------------------------------------------------------
1.  Made the changes  as described in the accompanying file:
Chris_S_suggestions.txt
--------------------------------------------------------------------------------
2. Made minor wording changes to decrase the length.
--------------------------------------------------------------------------------

